Obscuration-dependent evolution of Active Galactic Nuclei

We aim to constrain the evolution of AGN as a function of obscuration using an X-ray selected sample of $\sim2000$ AGN from a multi-tiered survey including the CDFS, AEGIS-XD, COSMOS and XMM-XXL fields. The spectra of individual X-ray sources are analysed using a Bayesian methodology with a physically realistic model to infer the posterior distribution of the hydrogen column density and intrinsic X-ray luminosity. We develop a novel non-parametric method which allows us to robustly infer the distribution of the AGN population in X-ray luminosity, redshift and obscuring column density, relying only on minimal smoothness assumptions. Our analysis properly incorporates uncertainties from low count spectra, photometric redshift measurements, association incompleteness and the limited sample size. We find that obscured AGN with $N_{H}>{\rm 10^{22}\, cm^{-2}}$ account for ${77}^{+4}_{-5}\%$ of the number density and luminosity density of the accretion SMBH population with $L_{{\rm X}}>10^{43}\text{ erg/s}$, averaged over cosmic time. Compton-thick AGN account for approximately half the number and luminosity density of the obscured population, and ${38}^{+8}_{-7}\%$ of the total. We also find evidence that the evolution is obscuration-dependent, with the strongest evolution around $N_{H}\thickapprox10^{23}\text{ cm}^{-2}$. We highlight this by measuring the obscured fraction in Compton-thin AGN, which increases towards $z\sim3$, where it is $25\%$ higher than the local value. In contrast the fraction of Compton-thick AGN is consistent with being constant at $\approx35\%$, independent of redshift and accretion luminosity. We discuss our findings in the context of existing models and conclude that the observed evolution is to first order a side-effect of anti-hierarchical growth.

==> fieldsummary.tex <==
\begin{tabular}{l l l | l}
$\log L$ & $z$ & $\log N_H$ & $\log \phi$ \\
\hline
42.0 - 42.4 & 0.001 - 0.1 & 20.0 - 21.0 & -4.88 - -4.26 \\
42.0 - 42.4 & 0.001 - 0.1 & 21.0 - 22.0 & -4.90 - -4.33 \\
42.0 - 42.4 & 0.001 - 0.1 & 22.0 - 23.0 & -4.79 - -4.15 \\
42.0 - 42.4 & 0.001 - 0.1 & 23.0 - 23.5 & -4.75 - -3.84 \\
42.0 - 42.4 & 0.001 - 0.1 & 23.5 - 24.0 & -4.85 - -3.66 \\
42.0 - 42.4 & 0.001 - 0.1 & 24.0 - 26.0 & -4.87 - -3.34 \\
42.0 - 42.4 & 0.1 - 0.3 & 20.0 - 21.0 & -4.80 - -4.32 \\
42.0 - 42.4 & 0.1 - 0.3 & 21.0 - 22.0 & -4.78 - -4.28 \\
42.0 - 42.4 & 0.1 - 0.3 & 22.0 - 23.0 & -4.62 - -4.09 \\
42.0 - 42.4 & 0.1 - 0.3 & 23.0 - 23.5 & -4.64 - -3.83 \\
42.0 - 42.4 & 0.1 - 0.3 & 23.5 - 24.0 & -4.78 - -3.69 \\
42.0 - 42.4 & 0.1 - 0.3 & 24.0 - 26.0 & -4.78 - -3.35 \\
42.0 - 42.4 & 0.3 - 0.5 & 20.0 - 21.0 & -4.71 - -4.32 \\
42.0 - 42.4 & 0.3 - 0.5 & 21.0 - 22.0 & -4.52 - -4.12 \\
42.0 - 42.4 & 0.3 - 0.5 & 22.0 - 23.0 & -4.30 - -3.90 \\
42.0 - 42.4 & 0.3 - 0.5 & 23.0 - 23.5 & -4.47 - -3.72 \\
42.0 - 42.4 & 0.3 - 0.5 & 23.5 - 24.0 & -4.71 - -3.63 \\
42.0 - 42.4 & 0.3 - 0.5 & 24.0 - 26.0 & -4.82 - -3.35 \\
42.0 - 42.4 & 0.5 - 0.75 & 20.0 - 21.0 & -4.70 - -4.32 \\
42.0 - 42.4 & 0.5 - 0.75 & 21.0 - 22.0 & -4.46 - -4.07 \\
42.0 - 42.4 & 0.5 - 0.75 & 22.0 - 23.0 & -4.14 - -3.78 \\
42.0 - 42.4 & 0.5 - 0.75 & 23.0 - 23.5 & -4.38 - -3.70 \\
42.0 - 42.4 & 0.5 - 0.75 & 23.5 - 24.0 & -4.65 - -3.60 \\
42.0 - 42.4 & 0.5 - 0.75 & 24.0 - 26.0 & -4.80 - -3.38 \\
42.0 - 42.4 & 0.75 - 1.0 & 20.0 - 21.0 & -4.74 - -4.29 \\
42.0 - 42.4 & 0.75 - 1.0 & 21.0 - 22.0 & -4.54 - -4.07 \\
42.0 - 42.4 & 0.75 - 1.0 & 22.0 - 23.0 & -4.29 - -3.86 \\
42.0 - 42.4 & 0.75 - 1.0 & 23.0 - 23.5 & -4.42 - -3.72 \\
42.0 - 42.4 & 0.75 - 1.0 & 23.5 - 24.0 & -4.65 - -3.58 \\
42.0 - 42.4 & 0.75 - 1.0 & 24.0 - 26.0 & -4.83 - -3.41 \\
42.0 - 42.4 & 1.0 - 1.25 & 20.0 - 21.0 & -4.79 - -4.20 \\
42.0 - 42.4 & 1.0 - 1.25 & 21.0 - 22.0 & -4.61 - -4.06 \\
42.0 - 42.4 & 1.0 - 1.25 & 22.0 - 23.0 & -4.42 - -3.90 \\
42.0 - 42.4 & 1.0 - 1.25 & 23.0 - 23.5 & -4.47 - -3.75 \\
42.0 - 42.4 & 1.0 - 1.25 & 23.5 - 24.0 & -4.69 - -3.60 \\
42.0 - 42.4 & 1.0 - 1.25 & 24.0 - 26.0 & -4.86 - -3.45 \\
42.0 - 42.4 & 1.25 - 1.5 & 20.0 - 21.0 & -4.81 - -4.10 \\
42.0 - 42.4 & 1.25 - 1.5 & 21.0 - 22.0 & -4.68 - -4.03 \\
42.0 - 42.4 & 1.25 - 1.5 & 22.0 - 23.0 & -4.55 - -3.93 \\
42.0 - 42.4 & 1.25 - 1.5 & 23.0 - 23.5 & -4.55 - -3.77 \\
42.0 - 42.4 & 1.25 - 1.5 & 23.5 - 24.0 & -4.75 - -3.61 \\
42.0 - 42.4 & 1.25 - 1.5 & 24.0 - 26.0 & -4.89 - -3.49 \\
42.0 - 42.4 & 1.5 - 1.8 & 20.0 - 21.0 & -4.91 - -4.01 \\
42.0 - 42.4 & 1.5 - 1.8 & 21.0 - 22.0 & -4.78 - -3.99 \\
42.0 - 42.4 & 1.5 - 1.8 & 22.0 - 23.0 & -4.67 - -3.92 \\
42.0 - 42.4 & 1.5 - 1.8 & 23.0 - 23.5 & -4.69 - -3.79 \\
42.0 - 42.4 & 1.5 - 1.8 & 23.5 - 24.0 & -4.81 - -3.66 \\
42.0 - 42.4 & 1.5 - 1.8 & 24.0 - 26.0 & -4.95 - -3.55 \\
42.0 - 42.4 & 1.8 - 2.1 & 20.0 - 21.0 & -4.99 - -3.93 \\
42.0 - 42.4 & 1.8 - 2.1 & 21.0 - 22.0 & -4.88 - -3.92 \\
42.0 - 42.4 & 1.8 - 2.1 & 22.0 - 23.0 & -4.81 - -3.88 \\
42.0 - 42.4 & 1.8 - 2.1 & 23.0 - 23.5 & -4.82 - -3.80 \\
42.0 - 42.4 & 1.8 - 2.1 & 23.5 - 24.0 & -4.93 - -3.70 \\
42.0 - 42.4 & 1.8 - 2.1 & 24.0 - 26.0 & -5.04 - -3.60 \\
42.0 - 42.4 & 2.1 - 2.7 & 20.0 - 21.0 & -5.07 - -3.91 \\
42.0 - 42.4 & 2.1 - 2.7 & 21.0 - 22.0 & -5.02 - -3.90 \\
42.0 - 42.4 & 2.1 - 2.7 & 22.0 - 23.0 & -4.94 - -3.88 \\
42.0 - 42.4 & 2.1 - 2.7 & 23.0 - 23.5 & -4.96 - -3.82 \\
42.0 - 42.4 & 2.1 - 2.7 & 23.5 - 24.0 & -5.04 - -3.75 \\
42.0 - 42.4 & 2.1 - 2.7 & 24.0 - 26.0 & -5.13 - -3.66 \\
42.0 - 42.4 & 2.7 - 3.2 & 20.0 - 21.0 & -5.20 - -3.86 \\
42.0 - 42.4 & 2.7 - 3.2 & 21.0 - 22.0 & -5.15 - -3.88 \\
42.0 - 42.4 & 2.7 - 3.2 & 22.0 - 23.0 & -5.10 - -3.89 \\
42.0 - 42.4 & 2.7 - 3.2 & 23.0 - 23.5 & -5.10 - -3.87 \\
42.0 - 42.4 & 2.7 - 3.2 & 23.5 - 24.0 & -5.16 - -3.81 \\
42.0 - 42.4 & 2.7 - 3.2 & 24.0 - 26.0 & -5.21 - -3.74 \\
42.0 - 42.4 & 3.2 - 4.0 & 20.0 - 21.0 & -5.32 - -3.88 \\
42.0 - 42.4 & 3.2 - 4.0 & 21.0 - 22.0 & -5.26 - -3.90 \\
42.0 - 42.4 & 3.2 - 4.0 & 22.0 - 23.0 & -5.22 - -3.92 \\
42.0 - 42.4 & 3.2 - 4.0 & 23.0 - 23.5 & -5.24 - -3.92 \\
42.0 - 42.4 & 3.2 - 4.0 & 23.5 - 24.0 & -5.25 - -3.88 \\
42.0 - 42.4 & 3.2 - 4.0 & 24.0 - 26.0 & -5.29 - -3.82 \\
42.0 - 42.4 & 4.0 - 7.0 & 20.0 - 21.0 & -5.39 - -3.96 \\
42.0 - 42.4 & 4.0 - 7.0 & 21.0 - 22.0 & -5.36 - -3.96 \\
42.0 - 42.4 & 4.0 - 7.0 & 22.0 - 23.0 & -5.31 - -4.00 \\
42.0 - 42.4 & 4.0 - 7.0 & 23.0 - 23.5 & -5.32 - -4.00 \\
42.0 - 42.4 & 4.0 - 7.0 & 23.5 - 24.0 & -5.32 - -3.97 \\
42.0 - 42.4 & 4.0 - 7.0 & 24.0 - 26.0 & -5.35 - -3.93 \\
\end{tabular}\newpage
\begin{tabular}{l l l | l}
$\log L$ & $z$ & $\log N_H$ & $\log \phi$ \\
\hline
42.4 - 42.8 & 0.001 - 0.1 & 20.0 - 21.0 & -4.98 - -4.61 \\
42.4 - 42.8 & 0.001 - 0.1 & 21.0 - 22.0 & -5.03 - -4.68 \\
42.4 - 42.8 & 0.001 - 0.1 & 22.0 - 23.0 & -4.92 - -4.54 \\
42.4 - 42.8 & 0.001 - 0.1 & 23.0 - 23.5 & -4.86 - -4.38 \\
42.4 - 42.8 & 0.001 - 0.1 & 23.5 - 24.0 & -4.95 - -4.25 \\
42.4 - 42.8 & 0.001 - 0.1 & 24.0 - 26.0 & -4.94 - -4.03 \\
42.4 - 42.8 & 0.1 - 0.3 & 20.0 - 21.0 & -4.85 - -4.56 \\
42.4 - 42.8 & 0.1 - 0.3 & 21.0 - 22.0 & -4.94 - -4.65 \\
42.4 - 42.8 & 0.1 - 0.3 & 22.0 - 23.0 & -4.82 - -4.49 \\
42.4 - 42.8 & 0.1 - 0.3 & 23.0 - 23.5 & -4.78 - -4.31 \\
42.4 - 42.8 & 0.1 - 0.3 & 23.5 - 24.0 & -4.88 - -4.22 \\
42.4 - 42.8 & 0.1 - 0.3 & 24.0 - 26.0 & -4.85 - -3.95 \\
42.4 - 42.8 & 0.3 - 0.5 & 20.0 - 21.0 & -4.73 - -4.45 \\
42.4 - 42.8 & 0.3 - 0.5 & 21.0 - 22.0 & -4.75 - -4.48 \\
42.4 - 42.8 & 0.3 - 0.5 & 22.0 - 23.0 & -4.59 - -4.30 \\
42.4 - 42.8 & 0.3 - 0.5 & 23.0 - 23.5 & -4.57 - -4.11 \\
42.4 - 42.8 & 0.3 - 0.5 & 23.5 - 24.0 & -4.74 - -4.07 \\
42.4 - 42.8 & 0.3 - 0.5 & 24.0 - 26.0 & -4.81 - -3.81 \\
42.4 - 42.8 & 0.5 - 0.75 & 20.0 - 21.0 & -4.67 - -4.41 \\
42.4 - 42.8 & 0.5 - 0.75 & 21.0 - 22.0 & -4.58 - -4.34 \\
42.4 - 42.8 & 0.5 - 0.75 & 22.0 - 23.0 & -4.36 - -4.12 \\
42.4 - 42.8 & 0.5 - 0.75 & 23.0 - 23.5 & -4.39 - -3.95 \\
42.4 - 42.8 & 0.5 - 0.75 & 23.5 - 24.0 & -4.66 - -3.96 \\
42.4 - 42.8 & 0.5 - 0.75 & 24.0 - 26.0 & -4.79 - -3.73 \\
42.4 - 42.8 & 0.75 - 1.0 & 20.0 - 21.0 & -4.76 - -4.43 \\
42.4 - 42.8 & 0.75 - 1.0 & 21.0 - 22.0 & -4.61 - -4.29 \\
42.4 - 42.8 & 0.75 - 1.0 & 22.0 - 23.0 & -4.30 - -3.98 \\
42.4 - 42.8 & 0.75 - 1.0 & 23.0 - 23.5 & -4.35 - -3.82 \\
42.4 - 42.8 & 0.75 - 1.0 & 23.5 - 24.0 & -4.64 - -3.88 \\
42.4 - 42.8 & 0.75 - 1.0 & 24.0 - 26.0 & -4.81 - -3.73 \\
42.4 - 42.8 & 1.0 - 1.25 & 20.0 - 21.0 & -4.83 - -4.43 \\
42.4 - 42.8 & 1.0 - 1.25 & 21.0 - 22.0 & -4.66 - -4.27 \\
42.4 - 42.8 & 1.0 - 1.25 & 22.0 - 23.0 & -4.35 - -3.96 \\
42.4 - 42.8 & 1.0 - 1.25 & 23.0 - 23.5 & -4.35 - -3.79 \\
42.4 - 42.8 & 1.0 - 1.25 & 23.5 - 24.0 & -4.65 - -3.82 \\
42.4 - 42.8 & 1.0 - 1.25 & 24.0 - 26.0 & -4.86 - -3.74 \\
42.4 - 42.8 & 1.25 - 1.5 & 20.0 - 21.0 & -4.85 - -4.38 \\
42.4 - 42.8 & 1.25 - 1.5 & 21.0 - 22.0 & -4.69 - -4.22 \\
42.4 - 42.8 & 1.25 - 1.5 & 22.0 - 23.0 & -4.49 - -4.00 \\
42.4 - 42.8 & 1.25 - 1.5 & 23.0 - 23.5 & -4.46 - -3.80 \\
42.4 - 42.8 & 1.25 - 1.5 & 23.5 - 24.0 & -4.71 - -3.81 \\
42.4 - 42.8 & 1.25 - 1.5 & 24.0 - 26.0 & -4.90 - -3.76 \\
42.4 - 42.8 & 1.5 - 1.8 & 20.0 - 21.0 & -4.90 - -4.31 \\
42.4 - 42.8 & 1.5 - 1.8 & 21.0 - 22.0 & -4.76 - -4.18 \\
42.4 - 42.8 & 1.5 - 1.8 & 22.0 - 23.0 & -4.60 - -4.02 \\
42.4 - 42.8 & 1.5 - 1.8 & 23.0 - 23.5 & -4.61 - -3.85 \\
42.4 - 42.8 & 1.5 - 1.8 & 23.5 - 24.0 & -4.79 - -3.84 \\
42.4 - 42.8 & 1.5 - 1.8 & 24.0 - 26.0 & -4.96 - -3.78 \\
42.4 - 42.8 & 1.8 - 2.1 & 20.0 - 21.0 & -4.98 - -4.25 \\
42.4 - 42.8 & 1.8 - 2.1 & 21.0 - 22.0 & -4.87 - -4.15 \\
42.4 - 42.8 & 1.8 - 2.1 & 22.0 - 23.0 & -4.75 - -4.05 \\
42.4 - 42.8 & 1.8 - 2.1 & 23.0 - 23.5 & -4.76 - -3.93 \\
42.4 - 42.8 & 1.8 - 2.1 & 23.5 - 24.0 & -4.90 - -3.88 \\
42.4 - 42.8 & 1.8 - 2.1 & 24.0 - 26.0 & -5.04 - -3.82 \\
42.4 - 42.8 & 2.1 - 2.7 & 20.0 - 21.0 & -5.09 - -4.24 \\
42.4 - 42.8 & 2.1 - 2.7 & 21.0 - 22.0 & -4.99 - -4.18 \\
42.4 - 42.8 & 2.1 - 2.7 & 22.0 - 23.0 & -4.93 - -4.09 \\
42.4 - 42.8 & 2.1 - 2.7 & 23.0 - 23.5 & -4.93 - -4.00 \\
42.4 - 42.8 & 2.1 - 2.7 & 23.5 - 24.0 & -5.00 - -3.95 \\
42.4 - 42.8 & 2.1 - 2.7 & 24.0 - 26.0 & -5.12 - -3.89 \\
42.4 - 42.8 & 2.7 - 3.2 & 20.0 - 21.0 & -5.21 - -4.26 \\
42.4 - 42.8 & 2.7 - 3.2 & 21.0 - 22.0 & -5.15 - -4.23 \\
42.4 - 42.8 & 2.7 - 3.2 & 22.0 - 23.0 & -5.09 - -4.17 \\
42.4 - 42.8 & 2.7 - 3.2 & 23.0 - 23.5 & -5.10 - -4.10 \\
42.4 - 42.8 & 2.7 - 3.2 & 23.5 - 24.0 & -5.17 - -4.06 \\
42.4 - 42.8 & 2.7 - 3.2 & 24.0 - 26.0 & -5.21 - -3.99 \\
42.4 - 42.8 & 3.2 - 4.0 & 20.0 - 21.0 & -5.33 - -4.31 \\
42.4 - 42.8 & 3.2 - 4.0 & 21.0 - 22.0 & -5.27 - -4.30 \\
42.4 - 42.8 & 3.2 - 4.0 & 22.0 - 23.0 & -5.22 - -4.26 \\
42.4 - 42.8 & 3.2 - 4.0 & 23.0 - 23.5 & -5.24 - -4.21 \\
42.4 - 42.8 & 3.2 - 4.0 & 23.5 - 24.0 & -5.26 - -4.16 \\
42.4 - 42.8 & 3.2 - 4.0 & 24.0 - 26.0 & -5.29 - -4.12 \\
42.4 - 42.8 & 4.0 - 7.0 & 20.0 - 21.0 & -5.41 - -4.43 \\
42.4 - 42.8 & 4.0 - 7.0 & 21.0 - 22.0 & -5.38 - -4.42 \\
42.4 - 42.8 & 4.0 - 7.0 & 22.0 - 23.0 & -5.33 - -4.41 \\
42.4 - 42.8 & 4.0 - 7.0 & 23.0 - 23.5 & -5.34 - -4.38 \\
42.4 - 42.8 & 4.0 - 7.0 & 23.5 - 24.0 & -5.34 - -4.32 \\
42.4 - 42.8 & 4.0 - 7.0 & 24.0 - 26.0 & -5.35 - -4.29 \\
\end{tabular}\newpage
\begin{tabular}{l l l | l}
$\log L$ & $z$ & $\log N_H$ & $\log \phi$ \\
\hline
42.8 - 43.2 & 0.001 - 0.1 & 20.0 - 21.0 & -5.26 - -4.90 \\
42.8 - 43.2 & 0.001 - 0.1 & 21.0 - 22.0 & -5.29 - -4.98 \\
42.8 - 43.2 & 0.001 - 0.1 & 22.0 - 23.0 & -5.18 - -4.87 \\
42.8 - 43.2 & 0.001 - 0.1 & 23.0 - 23.5 & -5.17 - -4.83 \\
42.8 - 43.2 & 0.001 - 0.1 & 23.5 - 24.0 & -5.14 - -4.77 \\
42.8 - 43.2 & 0.001 - 0.1 & 24.0 - 26.0 & -5.11 - -4.64 \\
42.8 - 43.2 & 0.1 - 0.3 & 20.0 - 21.0 & -5.12 - -4.87 \\
42.8 - 43.2 & 0.1 - 0.3 & 21.0 - 22.0 & -5.17 - -4.93 \\
42.8 - 43.2 & 0.1 - 0.3 & 22.0 - 23.0 & -4.97 - -4.71 \\
42.8 - 43.2 & 0.1 - 0.3 & 23.0 - 23.5 & -5.02 - -4.73 \\
42.8 - 43.2 & 0.1 - 0.3 & 23.5 - 24.0 & -5.05 - -4.71 \\
42.8 - 43.2 & 0.1 - 0.3 & 24.0 - 26.0 & -5.00 - -4.51 \\
42.8 - 43.2 & 0.3 - 0.5 & 20.0 - 21.0 & -4.89 - -4.63 \\
42.8 - 43.2 & 0.3 - 0.5 & 21.0 - 22.0 & -4.97 - -4.72 \\
42.8 - 43.2 & 0.3 - 0.5 & 22.0 - 23.0 & -4.81 - -4.57 \\
42.8 - 43.2 & 0.3 - 0.5 & 23.0 - 23.5 & -4.79 - -4.48 \\
42.8 - 43.2 & 0.3 - 0.5 & 23.5 - 24.0 & -4.90 - -4.50 \\
42.8 - 43.2 & 0.3 - 0.5 & 24.0 - 26.0 & -4.86 - -4.26 \\
42.8 - 43.2 & 0.5 - 0.75 & 20.0 - 21.0 & -4.69 - -4.47 \\
42.8 - 43.2 & 0.5 - 0.75 & 21.0 - 22.0 & -4.80 - -4.56 \\
42.8 - 43.2 & 0.5 - 0.75 & 22.0 - 23.0 & -4.46 - -4.27 \\
42.8 - 43.2 & 0.5 - 0.75 & 23.0 - 23.5 & -4.36 - -4.11 \\
42.8 - 43.2 & 0.5 - 0.75 & 23.5 - 24.0 & -4.70 - -4.29 \\
42.8 - 43.2 & 0.5 - 0.75 & 24.0 - 26.0 & -4.78 - -4.11 \\
42.8 - 43.2 & 0.75 - 1.0 & 20.0 - 21.0 & -4.73 - -4.50 \\
42.8 - 43.2 & 0.75 - 1.0 & 21.0 - 22.0 & -4.67 - -4.42 \\
42.8 - 43.2 & 0.75 - 1.0 & 22.0 - 23.0 & -4.17 - -3.95 \\
42.8 - 43.2 & 0.75 - 1.0 & 23.0 - 23.5 & -4.19 - -3.90 \\
42.8 - 43.2 & 0.75 - 1.0 & 23.5 - 24.0 & -4.65 - -4.14 \\
42.8 - 43.2 & 0.75 - 1.0 & 24.0 - 26.0 & -4.84 - -4.06 \\
42.8 - 43.2 & 1.0 - 1.25 & 20.0 - 21.0 & -4.81 - -4.56 \\
42.8 - 43.2 & 1.0 - 1.25 & 21.0 - 22.0 & -4.66 - -4.39 \\
42.8 - 43.2 & 1.0 - 1.25 & 22.0 - 23.0 & -4.16 - -3.95 \\
42.8 - 43.2 & 1.0 - 1.25 & 23.0 - 23.5 & -4.19 - -3.83 \\
42.8 - 43.2 & 1.0 - 1.25 & 23.5 - 24.0 & -4.63 - -4.05 \\
42.8 - 43.2 & 1.0 - 1.25 & 24.0 - 26.0 & -4.88 - -4.03 \\
42.8 - 43.2 & 1.25 - 1.5 & 20.0 - 21.0 & -4.88 - -4.57 \\
42.8 - 43.2 & 1.25 - 1.5 & 21.0 - 22.0 & -4.69 - -4.38 \\
42.8 - 43.2 & 1.25 - 1.5 & 22.0 - 23.0 & -4.35 - -4.04 \\
42.8 - 43.2 & 1.25 - 1.5 & 23.0 - 23.5 & -4.31 - -3.83 \\
42.8 - 43.2 & 1.25 - 1.5 & 23.5 - 24.0 & -4.67 - -3.99 \\
42.8 - 43.2 & 1.25 - 1.5 & 24.0 - 26.0 & -4.92 - -4.01 \\
42.8 - 43.2 & 1.5 - 1.8 & 20.0 - 21.0 & -4.91 - -4.53 \\
42.8 - 43.2 & 1.5 - 1.8 & 21.0 - 22.0 & -4.69 - -4.32 \\
42.8 - 43.2 & 1.5 - 1.8 & 22.0 - 23.0 & -4.43 - -4.09 \\
42.8 - 43.2 & 1.5 - 1.8 & 23.0 - 23.5 & -4.42 - -3.88 \\
42.8 - 43.2 & 1.5 - 1.8 & 23.5 - 24.0 & -4.73 - -3.98 \\
42.8 - 43.2 & 1.5 - 1.8 & 24.0 - 26.0 & -4.97 - -4.00 \\
42.8 - 43.2 & 1.8 - 2.1 & 20.0 - 21.0 & -5.01 - -4.53 \\
42.8 - 43.2 & 1.8 - 2.1 & 21.0 - 22.0 & -4.85 - -4.37 \\
42.8 - 43.2 & 1.8 - 2.1 & 22.0 - 23.0 & -4.67 - -4.20 \\
42.8 - 43.2 & 1.8 - 2.1 & 23.0 - 23.5 & -4.65 - -4.00 \\
42.8 - 43.2 & 1.8 - 2.1 & 23.5 - 24.0 & -4.86 - -4.03 \\
42.8 - 43.2 & 1.8 - 2.1 & 24.0 - 26.0 & -5.05 - -4.04 \\
42.8 - 43.2 & 2.1 - 2.7 & 20.0 - 21.0 & -5.14 - -4.55 \\
42.8 - 43.2 & 2.1 - 2.7 & 21.0 - 22.0 & -5.03 - -4.43 \\
42.8 - 43.2 & 2.1 - 2.7 & 22.0 - 23.0 & -4.88 - -4.28 \\
42.8 - 43.2 & 2.1 - 2.7 & 23.0 - 23.5 & -4.83 - -4.12 \\
42.8 - 43.2 & 2.1 - 2.7 & 23.5 - 24.0 & -4.98 - -4.11 \\
42.8 - 43.2 & 2.1 - 2.7 & 24.0 - 26.0 & -5.13 - -4.09 \\
42.8 - 43.2 & 2.7 - 3.2 & 20.0 - 21.0 & -5.29 - -4.60 \\
42.8 - 43.2 & 2.7 - 3.2 & 21.0 - 22.0 & -5.21 - -4.54 \\
42.8 - 43.2 & 2.7 - 3.2 & 22.0 - 23.0 & -5.10 - -4.42 \\
42.8 - 43.2 & 2.7 - 3.2 & 23.0 - 23.5 & -5.07 - -4.30 \\
42.8 - 43.2 & 2.7 - 3.2 & 23.5 - 24.0 & -5.14 - -4.27 \\
42.8 - 43.2 & 2.7 - 3.2 & 24.0 - 26.0 & -5.24 - -4.23 \\
42.8 - 43.2 & 3.2 - 4.0 & 20.0 - 21.0 & -5.40 - -4.69 \\
42.8 - 43.2 & 3.2 - 4.0 & 21.0 - 22.0 & -5.36 - -4.66 \\
42.8 - 43.2 & 3.2 - 4.0 & 22.0 - 23.0 & -5.29 - -4.56 \\
42.8 - 43.2 & 3.2 - 4.0 & 23.0 - 23.5 & -5.26 - -4.46 \\
42.8 - 43.2 & 3.2 - 4.0 & 23.5 - 24.0 & -5.28 - -4.42 \\
42.8 - 43.2 & 3.2 - 4.0 & 24.0 - 26.0 & -5.33 - -4.38 \\
42.8 - 43.2 & 4.0 - 7.0 & 20.0 - 21.0 & -5.51 - -4.87 \\
42.8 - 43.2 & 4.0 - 7.0 & 21.0 - 22.0 & -5.47 - -4.85 \\
42.8 - 43.2 & 4.0 - 7.0 & 22.0 - 23.0 & -5.42 - -4.79 \\
42.8 - 43.2 & 4.0 - 7.0 & 23.0 - 23.5 & -5.39 - -4.72 \\
42.8 - 43.2 & 4.0 - 7.0 & 23.5 - 24.0 & -5.39 - -4.66 \\
42.8 - 43.2 & 4.0 - 7.0 & 24.0 - 26.0 & -5.40 - -4.63 \\
\end{tabular}\newpage
\begin{tabular}{l l l | l}
$\log L$ & $z$ & $\log N_H$ & $\log \phi$ \\
\hline
43.2 - 43.6 & 0.001 - 0.1 & 20.0 - 21.0 & -5.64 - -5.25 \\
43.2 - 43.6 & 0.001 - 0.1 & 21.0 - 22.0 & -5.67 - -5.28 \\
43.2 - 43.6 & 0.001 - 0.1 & 22.0 - 23.0 & -5.61 - -5.21 \\
43.2 - 43.6 & 0.001 - 0.1 & 23.0 - 23.5 & -5.65 - -5.16 \\
43.2 - 43.6 & 0.001 - 0.1 & 23.5 - 24.0 & -5.58 - -5.12 \\
43.2 - 43.6 & 0.001 - 0.1 & 24.0 - 26.0 & -5.48 - -5.04 \\
43.2 - 43.6 & 0.1 - 0.3 & 20.0 - 21.0 & -5.47 - -5.20 \\
43.2 - 43.6 & 0.1 - 0.3 & 21.0 - 22.0 & -5.53 - -5.27 \\
43.2 - 43.6 & 0.1 - 0.3 & 22.0 - 23.0 & -5.44 - -5.17 \\
43.2 - 43.6 & 0.1 - 0.3 & 23.0 - 23.5 & -5.46 - -5.14 \\
43.2 - 43.6 & 0.1 - 0.3 & 23.5 - 24.0 & -5.44 - -5.10 \\
43.2 - 43.6 & 0.1 - 0.3 & 24.0 - 26.0 & -5.36 - -5.02 \\
43.2 - 43.6 & 0.3 - 0.5 & 20.0 - 21.0 & -5.26 - -5.00 \\
43.2 - 43.6 & 0.3 - 0.5 & 21.0 - 22.0 & -5.35 - -5.12 \\
43.2 - 43.6 & 0.3 - 0.5 & 22.0 - 23.0 & -5.24 - -5.01 \\
43.2 - 43.6 & 0.3 - 0.5 & 23.0 - 23.5 & -5.19 - -4.92 \\
43.2 - 43.6 & 0.3 - 0.5 & 23.5 - 24.0 & -5.23 - -4.96 \\
43.2 - 43.6 & 0.3 - 0.5 & 24.0 - 26.0 & -5.13 - -4.83 \\
43.2 - 43.6 & 0.5 - 0.75 & 20.0 - 21.0 & -5.04 - -4.82 \\
43.2 - 43.6 & 0.5 - 0.75 & 21.0 - 22.0 & -5.21 - -4.98 \\
43.2 - 43.6 & 0.5 - 0.75 & 22.0 - 23.0 & -4.96 - -4.74 \\
43.2 - 43.6 & 0.5 - 0.75 & 23.0 - 23.5 & -4.81 - -4.58 \\
43.2 - 43.6 & 0.5 - 0.75 & 23.5 - 24.0 & -5.02 - -4.76 \\
43.2 - 43.6 & 0.5 - 0.75 & 24.0 - 26.0 & -5.00 - -4.64 \\
43.2 - 43.6 & 0.75 - 1.0 & 20.0 - 21.0 & -5.10 - -4.84 \\
43.2 - 43.6 & 0.75 - 1.0 & 21.0 - 22.0 & -5.07 - -4.83 \\
43.2 - 43.6 & 0.75 - 1.0 & 22.0 - 23.0 & -4.77 - -4.54 \\
43.2 - 43.6 & 0.75 - 1.0 & 23.0 - 23.5 & -4.58 - -4.33 \\
43.2 - 43.6 & 0.75 - 1.0 & 23.5 - 24.0 & -4.94 - -4.59 \\
43.2 - 43.6 & 0.75 - 1.0 & 24.0 - 26.0 & -5.00 - -4.49 \\
43.2 - 43.6 & 1.0 - 1.25 & 20.0 - 21.0 & -5.01 - -4.78 \\
43.2 - 43.6 & 1.0 - 1.25 & 21.0 - 22.0 & -4.97 - -4.71 \\
43.2 - 43.6 & 1.0 - 1.25 & 22.0 - 23.0 & -4.52 - -4.34 \\
43.2 - 43.6 & 1.0 - 1.25 & 23.0 - 23.5 & -4.38 - -4.13 \\
43.2 - 43.6 & 1.0 - 1.25 & 23.5 - 24.0 & -4.83 - -4.42 \\
43.2 - 43.6 & 1.0 - 1.25 & 24.0 - 26.0 & -5.00 - -4.41 \\
43.2 - 43.6 & 1.25 - 1.5 & 20.0 - 21.0 & -5.05 - -4.78 \\
43.2 - 43.6 & 1.25 - 1.5 & 21.0 - 22.0 & -4.87 - -4.61 \\
43.2 - 43.6 & 1.25 - 1.5 & 22.0 - 23.0 & -4.52 - -4.29 \\
43.2 - 43.6 & 1.25 - 1.5 & 23.0 - 23.5 & -4.33 - -4.01 \\
43.2 - 43.6 & 1.25 - 1.5 & 23.5 - 24.0 & -4.73 - -4.26 \\
43.2 - 43.6 & 1.25 - 1.5 & 24.0 - 26.0 & -5.01 - -4.33 \\
43.2 - 43.6 & 1.5 - 1.8 & 20.0 - 21.0 & -5.07 - -4.78 \\
43.2 - 43.6 & 1.5 - 1.8 & 21.0 - 22.0 & -4.81 - -4.54 \\
43.2 - 43.6 & 1.5 - 1.8 & 22.0 - 23.0 & -4.50 - -4.27 \\
43.2 - 43.6 & 1.5 - 1.8 & 23.0 - 23.5 & -4.37 - -4.01 \\
43.2 - 43.6 & 1.5 - 1.8 & 23.5 - 24.0 & -4.70 - -4.19 \\
43.2 - 43.6 & 1.5 - 1.8 & 24.0 - 26.0 & -5.00 - -4.27 \\
43.2 - 43.6 & 1.8 - 2.1 & 20.0 - 21.0 & -5.14 - -4.79 \\
43.2 - 43.6 & 1.8 - 2.1 & 21.0 - 22.0 & -4.95 - -4.60 \\
43.2 - 43.6 & 1.8 - 2.1 & 22.0 - 23.0 & -4.75 - -4.41 \\
43.2 - 43.6 & 1.8 - 2.1 & 23.0 - 23.5 & -4.59 - -4.11 \\
43.2 - 43.6 & 1.8 - 2.1 & 23.5 - 24.0 & -4.82 - -4.22 \\
43.2 - 43.6 & 1.8 - 2.1 & 24.0 - 26.0 & -5.06 - -4.28 \\
43.2 - 43.6 & 2.1 - 2.7 & 20.0 - 21.0 & -5.26 - -4.84 \\
43.2 - 43.6 & 2.1 - 2.7 & 21.0 - 22.0 & -5.08 - -4.68 \\
43.2 - 43.6 & 2.1 - 2.7 & 22.0 - 23.0 & -4.88 - -4.50 \\
43.2 - 43.6 & 2.1 - 2.7 & 23.0 - 23.5 & -4.71 - -4.21 \\
43.2 - 43.6 & 2.1 - 2.7 & 23.5 - 24.0 & -4.96 - -4.30 \\
43.2 - 43.6 & 2.1 - 2.7 & 24.0 - 26.0 & -5.15 - -4.33 \\
43.2 - 43.6 & 2.7 - 3.2 & 20.0 - 21.0 & -5.42 - -4.92 \\
43.2 - 43.6 & 2.7 - 3.2 & 21.0 - 22.0 & -5.30 - -4.83 \\
43.2 - 43.6 & 2.7 - 3.2 & 22.0 - 23.0 & -5.15 - -4.68 \\
43.2 - 43.6 & 2.7 - 3.2 & 23.0 - 23.5 & -5.05 - -4.48 \\
43.2 - 43.6 & 2.7 - 3.2 & 23.5 - 24.0 & -5.16 - -4.47 \\
43.2 - 43.6 & 2.7 - 3.2 & 24.0 - 26.0 & -5.29 - -4.48 \\
43.2 - 43.6 & 3.2 - 4.0 & 20.0 - 21.0 & -5.56 - -5.07 \\
43.2 - 43.6 & 3.2 - 4.0 & 21.0 - 22.0 & -5.48 - -5.00 \\
43.2 - 43.6 & 3.2 - 4.0 & 22.0 - 23.0 & -5.39 - -4.87 \\
43.2 - 43.6 & 3.2 - 4.0 & 23.0 - 23.5 & -5.32 - -4.71 \\
43.2 - 43.6 & 3.2 - 4.0 & 23.5 - 24.0 & -5.34 - -4.66 \\
43.2 - 43.6 & 3.2 - 4.0 & 24.0 - 26.0 & -5.40 - -4.66 \\
43.2 - 43.6 & 4.0 - 7.0 & 20.0 - 21.0 & -5.69 - -5.30 \\
43.2 - 43.6 & 4.0 - 7.0 & 21.0 - 22.0 & -5.63 - -5.25 \\
43.2 - 43.6 & 4.0 - 7.0 & 22.0 - 23.0 & -5.56 - -5.17 \\
43.2 - 43.6 & 4.0 - 7.0 & 23.0 - 23.5 & -5.49 - -5.03 \\
43.2 - 43.6 & 4.0 - 7.0 & 23.5 - 24.0 & -5.48 - -4.99 \\
43.2 - 43.6 & 4.0 - 7.0 & 24.0 - 26.0 & -5.49 - -4.97 \\
\end{tabular}\newpage
\begin{tabular}{l l l | l}
$\log L$ & $z$ & $\log N_H$ & $\log \phi$ \\
\hline
43.6 - 44.0 & 0.001 - 0.1 & 20.0 - 21.0 & -6.14 - -5.59 \\
43.6 - 44.0 & 0.001 - 0.1 & 21.0 - 22.0 & -6.15 - -5.59 \\
43.6 - 44.0 & 0.001 - 0.1 & 22.0 - 23.0 & -6.13 - -5.52 \\
43.6 - 44.0 & 0.001 - 0.1 & 23.0 - 23.5 & -6.16 - -5.46 \\
43.6 - 44.0 & 0.001 - 0.1 & 23.5 - 24.0 & -6.14 - -5.41 \\
43.6 - 44.0 & 0.001 - 0.1 & 24.0 - 26.0 & -6.07 - -5.32 \\
43.6 - 44.0 & 0.1 - 0.3 & 20.0 - 21.0 & -5.96 - -5.61 \\
43.6 - 44.0 & 0.1 - 0.3 & 21.0 - 22.0 & -6.01 - -5.65 \\
43.6 - 44.0 & 0.1 - 0.3 & 22.0 - 23.0 & -5.98 - -5.56 \\
43.6 - 44.0 & 0.1 - 0.3 & 23.0 - 23.5 & -6.01 - -5.47 \\
43.6 - 44.0 & 0.1 - 0.3 & 23.5 - 24.0 & -5.98 - -5.44 \\
43.6 - 44.0 & 0.1 - 0.3 & 24.0 - 26.0 & -5.94 - -5.31 \\
43.6 - 44.0 & 0.3 - 0.5 & 20.0 - 21.0 & -5.64 - -5.43 \\
43.6 - 44.0 & 0.3 - 0.5 & 21.0 - 22.0 & -5.80 - -5.57 \\
43.6 - 44.0 & 0.3 - 0.5 & 22.0 - 23.0 & -5.72 - -5.48 \\
43.6 - 44.0 & 0.3 - 0.5 & 23.0 - 23.5 & -5.71 - -5.40 \\
43.6 - 44.0 & 0.3 - 0.5 & 23.5 - 24.0 & -5.73 - -5.36 \\
43.6 - 44.0 & 0.3 - 0.5 & 24.0 - 26.0 & -5.68 - -5.25 \\
43.6 - 44.0 & 0.5 - 0.75 & 20.0 - 21.0 & -5.55 - -5.32 \\
43.6 - 44.0 & 0.5 - 0.75 & 21.0 - 22.0 & -5.70 - -5.46 \\
43.6 - 44.0 & 0.5 - 0.75 & 22.0 - 23.0 & -5.53 - -5.32 \\
43.6 - 44.0 & 0.5 - 0.75 & 23.0 - 23.5 & -5.44 - -5.16 \\
43.6 - 44.0 & 0.5 - 0.75 & 23.5 - 24.0 & -5.52 - -5.22 \\
43.6 - 44.0 & 0.5 - 0.75 & 24.0 - 26.0 & -5.45 - -5.14 \\
43.6 - 44.0 & 0.75 - 1.0 & 20.0 - 21.0 & -5.34 - -5.10 \\
43.6 - 44.0 & 0.75 - 1.0 & 21.0 - 22.0 & -5.44 - -5.22 \\
43.6 - 44.0 & 0.75 - 1.0 & 22.0 - 23.0 & -5.22 - -5.01 \\
43.6 - 44.0 & 0.75 - 1.0 & 23.0 - 23.5 & -5.16 - -4.92 \\
43.6 - 44.0 & 0.75 - 1.0 & 23.5 - 24.0 & -5.32 - -5.08 \\
43.6 - 44.0 & 0.75 - 1.0 & 24.0 - 26.0 & -5.28 - -4.99 \\
43.6 - 44.0 & 1.0 - 1.25 & 20.0 - 21.0 & -5.24 - -5.00 \\
43.6 - 44.0 & 1.0 - 1.25 & 21.0 - 22.0 & -5.29 - -5.05 \\
43.6 - 44.0 & 1.0 - 1.25 & 22.0 - 23.0 & -5.05 - -4.85 \\
43.6 - 44.0 & 1.0 - 1.25 & 23.0 - 23.5 & -4.86 - -4.64 \\
43.6 - 44.0 & 1.0 - 1.25 & 23.5 - 24.0 & -5.16 - -4.87 \\
43.6 - 44.0 & 1.0 - 1.25 & 24.0 - 26.0 & -5.23 - -4.88 \\
43.6 - 44.0 & 1.25 - 1.5 & 20.0 - 21.0 & -5.26 - -4.99 \\
43.6 - 44.0 & 1.25 - 1.5 & 21.0 - 22.0 & -5.17 - -4.91 \\
43.6 - 44.0 & 1.25 - 1.5 & 22.0 - 23.0 & -4.96 - -4.73 \\
43.6 - 44.0 & 1.25 - 1.5 & 23.0 - 23.5 & -4.65 - -4.41 \\
43.6 - 44.0 & 1.25 - 1.5 & 23.5 - 24.0 & -4.99 - -4.67 \\
43.6 - 44.0 & 1.25 - 1.5 & 24.0 - 26.0 & -5.19 - -4.73 \\
43.6 - 44.0 & 1.5 - 1.8 & 20.0 - 21.0 & -5.21 - -4.95 \\
43.6 - 44.0 & 1.5 - 1.8 & 21.0 - 22.0 & -4.98 - -4.76 \\
43.6 - 44.0 & 1.5 - 1.8 & 22.0 - 23.0 & -4.79 - -4.59 \\
43.6 - 44.0 & 1.5 - 1.8 & 23.0 - 23.5 & -4.48 - -4.26 \\
43.6 - 44.0 & 1.5 - 1.8 & 23.5 - 24.0 & -4.84 - -4.51 \\
43.6 - 44.0 & 1.5 - 1.8 & 24.0 - 26.0 & -5.10 - -4.61 \\
43.6 - 44.0 & 1.8 - 2.1 & 20.0 - 21.0 & -5.29 - -5.00 \\
43.6 - 44.0 & 1.8 - 2.1 & 21.0 - 22.0 & -5.11 - -4.83 \\
43.6 - 44.0 & 1.8 - 2.1 & 22.0 - 23.0 & -4.92 - -4.66 \\
43.6 - 44.0 & 1.8 - 2.1 & 23.0 - 23.5 & -4.66 - -4.31 \\
43.6 - 44.0 & 1.8 - 2.1 & 23.5 - 24.0 & -4.90 - -4.46 \\
43.6 - 44.0 & 1.8 - 2.1 & 24.0 - 26.0 & -5.11 - -4.56 \\
43.6 - 44.0 & 2.1 - 2.7 & 20.0 - 21.0 & -5.43 - -5.09 \\
43.6 - 44.0 & 2.1 - 2.7 & 21.0 - 22.0 & -5.25 - -4.93 \\
43.6 - 44.0 & 2.1 - 2.7 & 22.0 - 23.0 & -4.99 - -4.73 \\
43.6 - 44.0 & 2.1 - 2.7 & 23.0 - 23.5 & -4.73 - -4.41 \\
43.6 - 44.0 & 2.1 - 2.7 & 23.5 - 24.0 & -4.99 - -4.53 \\
43.6 - 44.0 & 2.1 - 2.7 & 24.0 - 26.0 & -5.18 - -4.61 \\
43.6 - 44.0 & 2.7 - 3.2 & 20.0 - 21.0 & -5.59 - -5.25 \\
43.6 - 44.0 & 2.7 - 3.2 & 21.0 - 22.0 & -5.50 - -5.15 \\
43.6 - 44.0 & 2.7 - 3.2 & 22.0 - 23.0 & -5.29 - -4.94 \\
43.6 - 44.0 & 2.7 - 3.2 & 23.0 - 23.5 & -5.09 - -4.67 \\
43.6 - 44.0 & 2.7 - 3.2 & 23.5 - 24.0 & -5.20 - -4.70 \\
43.6 - 44.0 & 2.7 - 3.2 & 24.0 - 26.0 & -5.36 - -4.76 \\
43.6 - 44.0 & 3.2 - 4.0 & 20.0 - 21.0 & -5.77 - -5.41 \\
43.6 - 44.0 & 3.2 - 4.0 & 21.0 - 22.0 & -5.67 - -5.35 \\
43.6 - 44.0 & 3.2 - 4.0 & 22.0 - 23.0 & -5.55 - -5.19 \\
43.6 - 44.0 & 3.2 - 4.0 & 23.0 - 23.5 & -5.42 - -4.98 \\
43.6 - 44.0 & 3.2 - 4.0 & 23.5 - 24.0 & -5.46 - -4.94 \\
43.6 - 44.0 & 3.2 - 4.0 & 24.0 - 26.0 & -5.52 - -4.98 \\
43.6 - 44.0 & 4.0 - 7.0 & 20.0 - 21.0 & -5.97 - -5.63 \\
43.6 - 44.0 & 4.0 - 7.0 & 21.0 - 22.0 & -5.89 - -5.60 \\
43.6 - 44.0 & 4.0 - 7.0 & 22.0 - 23.0 & -5.78 - -5.51 \\
43.6 - 44.0 & 4.0 - 7.0 & 23.0 - 23.5 & -5.68 - -5.36 \\
43.6 - 44.0 & 4.0 - 7.0 & 23.5 - 24.0 & -5.65 - -5.32 \\
43.6 - 44.0 & 4.0 - 7.0 & 24.0 - 26.0 & -5.66 - -5.33 \\
\end{tabular}\newpage
\begin{tabular}{l l l | l}
$\log L$ & $z$ & $\log N_H$ & $\log \phi$ \\
\hline
44.0 - 44.4 & 0.001 - 0.1 & 20.0 - 21.0 & -6.72 - -5.86 \\
44.0 - 44.4 & 0.001 - 0.1 & 21.0 - 22.0 & -6.70 - -5.87 \\
44.0 - 44.4 & 0.001 - 0.1 & 22.0 - 23.0 & -6.70 - -5.81 \\
44.0 - 44.4 & 0.001 - 0.1 & 23.0 - 23.5 & -6.72 - -5.74 \\
44.0 - 44.4 & 0.001 - 0.1 & 23.5 - 24.0 & -6.71 - -5.67 \\
44.0 - 44.4 & 0.001 - 0.1 & 24.0 - 26.0 & -6.69 - -5.61 \\
44.0 - 44.4 & 0.1 - 0.3 & 20.0 - 21.0 & -6.54 - -5.91 \\
44.0 - 44.4 & 0.1 - 0.3 & 21.0 - 22.0 & -6.57 - -5.91 \\
44.0 - 44.4 & 0.1 - 0.3 & 22.0 - 23.0 & -6.57 - -5.88 \\
44.0 - 44.4 & 0.1 - 0.3 & 23.0 - 23.5 & -6.58 - -5.79 \\
44.0 - 44.4 & 0.1 - 0.3 & 23.5 - 24.0 & -6.59 - -5.72 \\
44.0 - 44.4 & 0.1 - 0.3 & 24.0 - 26.0 & -6.56 - -5.60 \\
44.0 - 44.4 & 0.3 - 0.5 & 20.0 - 21.0 & -6.22 - -5.86 \\
44.0 - 44.4 & 0.3 - 0.5 & 21.0 - 22.0 & -6.34 - -5.94 \\
44.0 - 44.4 & 0.3 - 0.5 & 22.0 - 23.0 & -6.35 - -5.88 \\
44.0 - 44.4 & 0.3 - 0.5 & 23.0 - 23.5 & -6.34 - -5.78 \\
44.0 - 44.4 & 0.3 - 0.5 & 23.5 - 24.0 & -6.35 - -5.69 \\
44.0 - 44.4 & 0.3 - 0.5 & 24.0 - 26.0 & -6.33 - -5.56 \\
44.0 - 44.4 & 0.5 - 0.75 & 20.0 - 21.0 & -5.93 - -5.70 \\
44.0 - 44.4 & 0.5 - 0.75 & 21.0 - 22.0 & -6.14 - -5.86 \\
44.0 - 44.4 & 0.5 - 0.75 & 22.0 - 23.0 & -6.13 - -5.84 \\
44.0 - 44.4 & 0.5 - 0.75 & 23.0 - 23.5 & -6.10 - -5.72 \\
44.0 - 44.4 & 0.5 - 0.75 & 23.5 - 24.0 & -6.14 - -5.63 \\
44.0 - 44.4 & 0.5 - 0.75 & 24.0 - 26.0 & -6.09 - -5.50 \\
44.0 - 44.4 & 0.75 - 1.0 & 20.0 - 21.0 & -5.73 - -5.48 \\
44.0 - 44.4 & 0.75 - 1.0 & 21.0 - 22.0 & -5.92 - -5.66 \\
44.0 - 44.4 & 0.75 - 1.0 & 22.0 - 23.0 & -5.86 - -5.60 \\
44.0 - 44.4 & 0.75 - 1.0 & 23.0 - 23.5 & -5.80 - -5.51 \\
44.0 - 44.4 & 0.75 - 1.0 & 23.5 - 24.0 & -5.87 - -5.53 \\
44.0 - 44.4 & 0.75 - 1.0 & 24.0 - 26.0 & -5.83 - -5.40 \\
44.0 - 44.4 & 1.0 - 1.25 & 20.0 - 21.0 & -5.62 - -5.36 \\
44.0 - 44.4 & 1.0 - 1.25 & 21.0 - 22.0 & -5.74 - -5.49 \\
44.0 - 44.4 & 1.0 - 1.25 & 22.0 - 23.0 & -5.65 - -5.42 \\
44.0 - 44.4 & 1.0 - 1.25 & 23.0 - 23.5 & -5.51 - -5.26 \\
44.0 - 44.4 & 1.0 - 1.25 & 23.5 - 24.0 & -5.64 - -5.38 \\
44.0 - 44.4 & 1.0 - 1.25 & 24.0 - 26.0 & -5.61 - -5.30 \\
44.0 - 44.4 & 1.25 - 1.5 & 20.0 - 21.0 & -5.50 - -5.23 \\
44.0 - 44.4 & 1.25 - 1.5 & 21.0 - 22.0 & -5.52 - -5.26 \\
44.0 - 44.4 & 1.25 - 1.5 & 22.0 - 23.0 & -5.43 - -5.19 \\
44.0 - 44.4 & 1.25 - 1.5 & 23.0 - 23.5 & -5.29 - -5.00 \\
44.0 - 44.4 & 1.25 - 1.5 & 23.5 - 24.0 & -5.44 - -5.18 \\
44.0 - 44.4 & 1.25 - 1.5 & 24.0 - 26.0 & -5.49 - -5.17 \\
44.0 - 44.4 & 1.5 - 1.8 & 20.0 - 21.0 & -5.42 - -5.14 \\
44.0 - 44.4 & 1.5 - 1.8 & 21.0 - 22.0 & -5.32 - -5.08 \\
44.0 - 44.4 & 1.5 - 1.8 & 22.0 - 23.0 & -5.21 - -4.99 \\
44.0 - 44.4 & 1.5 - 1.8 & 23.0 - 23.5 & -5.07 - -4.80 \\
44.0 - 44.4 & 1.5 - 1.8 & 23.5 - 24.0 & -5.23 - -4.96 \\
44.0 - 44.4 & 1.5 - 1.8 & 24.0 - 26.0 & -5.30 - -5.00 \\
44.0 - 44.4 & 1.8 - 2.1 & 20.0 - 21.0 & -5.40 - -5.13 \\
44.0 - 44.4 & 1.8 - 2.1 & 21.0 - 22.0 & -5.34 - -5.08 \\
44.0 - 44.4 & 1.8 - 2.1 & 22.0 - 23.0 & -5.20 - -4.96 \\
44.0 - 44.4 & 1.8 - 2.1 & 23.0 - 23.5 & -5.03 - -4.72 \\
44.0 - 44.4 & 1.8 - 2.1 & 23.5 - 24.0 & -5.16 - -4.87 \\
44.0 - 44.4 & 1.8 - 2.1 & 24.0 - 26.0 & -5.24 - -4.92 \\
44.0 - 44.4 & 2.1 - 2.7 & 20.0 - 21.0 & -5.58 - -5.29 \\
44.0 - 44.4 & 2.1 - 2.7 & 21.0 - 22.0 & -5.44 - -5.19 \\
44.0 - 44.4 & 2.1 - 2.7 & 22.0 - 23.0 & -5.16 - -4.94 \\
44.0 - 44.4 & 2.1 - 2.7 & 23.0 - 23.5 & -4.92 - -4.69 \\
44.0 - 44.4 & 2.1 - 2.7 & 23.5 - 24.0 & -5.13 - -4.86 \\
44.0 - 44.4 & 2.1 - 2.7 & 24.0 - 26.0 & -5.25 - -4.94 \\
44.0 - 44.4 & 2.7 - 3.2 & 20.0 - 21.0 & -5.85 - -5.55 \\
44.0 - 44.4 & 2.7 - 3.2 & 21.0 - 22.0 & -5.71 - -5.43 \\
44.0 - 44.4 & 2.7 - 3.2 & 22.0 - 23.0 & -5.48 - -5.22 \\
44.0 - 44.4 & 2.7 - 3.2 & 23.0 - 23.5 & -5.22 - -4.95 \\
44.0 - 44.4 & 2.7 - 3.2 & 23.5 - 24.0 & -5.35 - -5.03 \\
44.0 - 44.4 & 2.7 - 3.2 & 24.0 - 26.0 & -5.47 - -5.12 \\
44.0 - 44.4 & 3.2 - 4.0 & 20.0 - 21.0 & -6.04 - -5.75 \\
44.0 - 44.4 & 3.2 - 4.0 & 21.0 - 22.0 & -5.93 - -5.68 \\
44.0 - 44.4 & 3.2 - 4.0 & 22.0 - 23.0 & -5.79 - -5.51 \\
44.0 - 44.4 & 3.2 - 4.0 & 23.0 - 23.5 & -5.61 - -5.31 \\
44.0 - 44.4 & 3.2 - 4.0 & 23.5 - 24.0 & -5.62 - -5.31 \\
44.0 - 44.4 & 3.2 - 4.0 & 24.0 - 26.0 & -5.67 - -5.36 \\
44.0 - 44.4 & 4.0 - 7.0 & 20.0 - 21.0 & -6.36 - -5.93 \\
44.0 - 44.4 & 4.0 - 7.0 & 21.0 - 22.0 & -6.26 - -5.89 \\
44.0 - 44.4 & 4.0 - 7.0 & 22.0 - 23.0 & -6.13 - -5.81 \\
44.0 - 44.4 & 4.0 - 7.0 & 23.0 - 23.5 & -5.99 - -5.66 \\
44.0 - 44.4 & 4.0 - 7.0 & 23.5 - 24.0 & -5.98 - -5.62 \\
44.0 - 44.4 & 4.0 - 7.0 & 24.0 - 26.0 & -6.00 - -5.60 \\
\end{tabular}\newpage
\begin{tabular}{l l l | l}
$\log L$ & $z$ & $\log N_H$ & $\log \phi$ \\
\hline
44.4 - 44.8 & 0.001 - 0.1 & 20.0 - 21.0 & -7.32 - -6.12 \\
44.4 - 44.8 & 0.001 - 0.1 & 21.0 - 22.0 & -7.28 - -6.10 \\
44.4 - 44.8 & 0.001 - 0.1 & 22.0 - 23.0 & -7.28 - -6.07 \\
44.4 - 44.8 & 0.001 - 0.1 & 23.0 - 23.5 & -7.29 - -5.98 \\
44.4 - 44.8 & 0.001 - 0.1 & 23.5 - 24.0 & -7.28 - -5.93 \\
44.4 - 44.8 & 0.001 - 0.1 & 24.0 - 26.0 & -7.29 - -5.85 \\
44.4 - 44.8 & 0.1 - 0.3 & 20.0 - 21.0 & -7.15 - -6.19 \\
44.4 - 44.8 & 0.1 - 0.3 & 21.0 - 22.0 & -7.16 - -6.19 \\
44.4 - 44.8 & 0.1 - 0.3 & 22.0 - 23.0 & -7.18 - -6.15 \\
44.4 - 44.8 & 0.1 - 0.3 & 23.0 - 23.5 & -7.18 - -6.05 \\
44.4 - 44.8 & 0.1 - 0.3 & 23.5 - 24.0 & -7.18 - -5.99 \\
44.4 - 44.8 & 0.1 - 0.3 & 24.0 - 26.0 & -7.18 - -5.88 \\
44.4 - 44.8 & 0.3 - 0.5 & 20.0 - 21.0 & -6.86 - -6.22 \\
44.4 - 44.8 & 0.3 - 0.5 & 21.0 - 22.0 & -6.96 - -6.27 \\
44.4 - 44.8 & 0.3 - 0.5 & 22.0 - 23.0 & -6.98 - -6.24 \\
44.4 - 44.8 & 0.3 - 0.5 & 23.0 - 23.5 & -6.99 - -6.11 \\
44.4 - 44.8 & 0.3 - 0.5 & 23.5 - 24.0 & -6.98 - -6.02 \\
44.4 - 44.8 & 0.3 - 0.5 & 24.0 - 26.0 & -6.97 - -5.87 \\
44.4 - 44.8 & 0.5 - 0.75 & 20.0 - 21.0 & -6.57 - -6.19 \\
44.4 - 44.8 & 0.5 - 0.75 & 21.0 - 22.0 & -6.74 - -6.32 \\
44.4 - 44.8 & 0.5 - 0.75 & 22.0 - 23.0 & -6.81 - -6.32 \\
44.4 - 44.8 & 0.5 - 0.75 & 23.0 - 23.5 & -6.78 - -6.12 \\
44.4 - 44.8 & 0.5 - 0.75 & 23.5 - 24.0 & -6.78 - -6.05 \\
44.4 - 44.8 & 0.5 - 0.75 & 24.0 - 26.0 & -6.75 - -5.88 \\
44.4 - 44.8 & 0.75 - 1.0 & 20.0 - 21.0 & -6.27 - -6.03 \\
44.4 - 44.8 & 0.75 - 1.0 & 21.0 - 22.0 & -6.50 - -6.21 \\
44.4 - 44.8 & 0.75 - 1.0 & 22.0 - 23.0 & -6.57 - -6.25 \\
44.4 - 44.8 & 0.75 - 1.0 & 23.0 - 23.5 & -6.51 - -6.05 \\
44.4 - 44.8 & 0.75 - 1.0 & 23.5 - 24.0 & -6.54 - -5.98 \\
44.4 - 44.8 & 0.75 - 1.0 & 24.0 - 26.0 & -6.51 - -5.85 \\
44.4 - 44.8 & 1.0 - 1.25 & 20.0 - 21.0 & -6.16 - -5.91 \\
44.4 - 44.8 & 1.0 - 1.25 & 21.0 - 22.0 & -6.34 - -6.10 \\
44.4 - 44.8 & 1.0 - 1.25 & 22.0 - 23.0 & -6.36 - -6.11 \\
44.4 - 44.8 & 1.0 - 1.25 & 23.0 - 23.5 & -6.24 - -5.92 \\
44.4 - 44.8 & 1.0 - 1.25 & 23.5 - 24.0 & -6.28 - -5.88 \\
44.4 - 44.8 & 1.0 - 1.25 & 24.0 - 26.0 & -6.26 - -5.77 \\
44.4 - 44.8 & 1.25 - 1.5 & 20.0 - 21.0 & -5.98 - -5.70 \\
44.4 - 44.8 & 1.25 - 1.5 & 21.0 - 22.0 & -6.12 - -5.84 \\
44.4 - 44.8 & 1.25 - 1.5 & 22.0 - 23.0 & -6.12 - -5.87 \\
44.4 - 44.8 & 1.25 - 1.5 & 23.0 - 23.5 & -6.01 - -5.74 \\
44.4 - 44.8 & 1.25 - 1.5 & 23.5 - 24.0 & -6.05 - -5.76 \\
44.4 - 44.8 & 1.25 - 1.5 & 24.0 - 26.0 & -6.06 - -5.69 \\
44.4 - 44.8 & 1.5 - 1.8 & 20.0 - 21.0 & -5.85 - -5.58 \\
44.4 - 44.8 & 1.5 - 1.8 & 21.0 - 22.0 & -5.93 - -5.68 \\
44.4 - 44.8 & 1.5 - 1.8 & 22.0 - 23.0 & -5.94 - -5.70 \\
44.4 - 44.8 & 1.5 - 1.8 & 23.0 - 23.5 & -5.82 - -5.56 \\
44.4 - 44.8 & 1.5 - 1.8 & 23.5 - 24.0 & -5.87 - -5.63 \\
44.4 - 44.8 & 1.5 - 1.8 & 24.0 - 26.0 & -5.87 - -5.56 \\
44.4 - 44.8 & 1.8 - 2.1 & 20.0 - 21.0 & -5.92 - -5.60 \\
44.4 - 44.8 & 1.8 - 2.1 & 21.0 - 22.0 & -5.92 - -5.65 \\
44.4 - 44.8 & 1.8 - 2.1 & 22.0 - 23.0 & -5.90 - -5.62 \\
44.4 - 44.8 & 1.8 - 2.1 & 23.0 - 23.5 & -5.75 - -5.48 \\
44.4 - 44.8 & 1.8 - 2.1 & 23.5 - 24.0 & -5.80 - -5.53 \\
44.4 - 44.8 & 1.8 - 2.1 & 24.0 - 26.0 & -5.78 - -5.50 \\
44.4 - 44.8 & 2.1 - 2.7 & 20.0 - 21.0 & -5.99 - -5.72 \\
44.4 - 44.8 & 2.1 - 2.7 & 21.0 - 22.0 & -5.96 - -5.73 \\
44.4 - 44.8 & 2.1 - 2.7 & 22.0 - 23.0 & -5.86 - -5.63 \\
44.4 - 44.8 & 2.1 - 2.7 & 23.0 - 23.5 & -5.75 - -5.50 \\
44.4 - 44.8 & 2.1 - 2.7 & 23.5 - 24.0 & -5.80 - -5.56 \\
44.4 - 44.8 & 2.1 - 2.7 & 24.0 - 26.0 & -5.77 - -5.52 \\
44.4 - 44.8 & 2.7 - 3.2 & 20.0 - 21.0 & -6.24 - -5.93 \\
44.4 - 44.8 & 2.7 - 3.2 & 21.0 - 22.0 & -6.14 - -5.88 \\
44.4 - 44.8 & 2.7 - 3.2 & 22.0 - 23.0 & -5.97 - -5.72 \\
44.4 - 44.8 & 2.7 - 3.2 & 23.0 - 23.5 & -5.81 - -5.55 \\
44.4 - 44.8 & 2.7 - 3.2 & 23.5 - 24.0 & -5.87 - -5.60 \\
44.4 - 44.8 & 2.7 - 3.2 & 24.0 - 26.0 & -5.88 - -5.57 \\
44.4 - 44.8 & 3.2 - 4.0 & 20.0 - 21.0 & -6.48 - -6.13 \\
44.4 - 44.8 & 3.2 - 4.0 & 21.0 - 22.0 & -6.36 - -6.05 \\
44.4 - 44.8 & 3.2 - 4.0 & 22.0 - 23.0 & -6.19 - -5.90 \\
44.4 - 44.8 & 3.2 - 4.0 & 23.0 - 23.5 & -6.06 - -5.79 \\
44.4 - 44.8 & 3.2 - 4.0 & 23.5 - 24.0 & -6.10 - -5.80 \\
44.4 - 44.8 & 3.2 - 4.0 & 24.0 - 26.0 & -6.11 - -5.73 \\
44.4 - 44.8 & 4.0 - 7.0 & 20.0 - 21.0 & -6.82 - -6.27 \\
44.4 - 44.8 & 4.0 - 7.0 & 21.0 - 22.0 & -6.74 - -6.22 \\
44.4 - 44.8 & 4.0 - 7.0 & 22.0 - 23.0 & -6.60 - -6.14 \\
44.4 - 44.8 & 4.0 - 7.0 & 23.0 - 23.5 & -6.49 - -6.01 \\
44.4 - 44.8 & 4.0 - 7.0 & 23.5 - 24.0 & -6.50 - -5.96 \\
44.4 - 44.8 & 4.0 - 7.0 & 24.0 - 26.0 & -6.51 - -5.90 \\
\end{tabular}\newpage
\begin{tabular}{l l l | l}
$\log L$ & $z$ & $\log N_H$ & $\log \phi$ \\
\hline
44.8 - 45.2 & 0.001 - 0.1 & 20.0 - 21.0 & -7.93 - -6.31 \\
44.8 - 45.2 & 0.001 - 0.1 & 21.0 - 22.0 & -7.89 - -6.29 \\
44.8 - 45.2 & 0.001 - 0.1 & 22.0 - 23.0 & -7.88 - -6.24 \\
44.8 - 45.2 & 0.001 - 0.1 & 23.0 - 23.5 & -7.90 - -6.19 \\
44.8 - 45.2 & 0.001 - 0.1 & 23.5 - 24.0 & -7.90 - -6.14 \\
44.8 - 45.2 & 0.001 - 0.1 & 24.0 - 26.0 & -7.90 - -6.06 \\
44.8 - 45.2 & 0.1 - 0.3 & 20.0 - 21.0 & -7.79 - -6.39 \\
44.8 - 45.2 & 0.1 - 0.3 & 21.0 - 22.0 & -7.78 - -6.35 \\
44.8 - 45.2 & 0.1 - 0.3 & 22.0 - 23.0 & -7.79 - -6.34 \\
44.8 - 45.2 & 0.1 - 0.3 & 23.0 - 23.5 & -7.79 - -6.26 \\
44.8 - 45.2 & 0.1 - 0.3 & 23.5 - 24.0 & -7.80 - -6.21 \\
44.8 - 45.2 & 0.1 - 0.3 & 24.0 - 26.0 & -7.80 - -6.12 \\
44.8 - 45.2 & 0.3 - 0.5 & 20.0 - 21.0 & -7.52 - -6.45 \\
44.8 - 45.2 & 0.3 - 0.5 & 21.0 - 22.0 & -7.59 - -6.48 \\
44.8 - 45.2 & 0.3 - 0.5 & 22.0 - 23.0 & -7.61 - -6.44 \\
44.8 - 45.2 & 0.3 - 0.5 & 23.0 - 23.5 & -7.62 - -6.33 \\
44.8 - 45.2 & 0.3 - 0.5 & 23.5 - 24.0 & -7.62 - -6.25 \\
44.8 - 45.2 & 0.3 - 0.5 & 24.0 - 26.0 & -7.62 - -6.13 \\
44.8 - 45.2 & 0.5 - 0.75 & 20.0 - 21.0 & -7.28 - -6.52 \\
44.8 - 45.2 & 0.5 - 0.75 & 21.0 - 22.0 & -7.39 - -6.55 \\
44.8 - 45.2 & 0.5 - 0.75 & 22.0 - 23.0 & -7.46 - -6.54 \\
44.8 - 45.2 & 0.5 - 0.75 & 23.0 - 23.5 & -7.44 - -6.37 \\
44.8 - 45.2 & 0.5 - 0.75 & 23.5 - 24.0 & -7.43 - -6.30 \\
44.8 - 45.2 & 0.5 - 0.75 & 24.0 - 26.0 & -7.42 - -6.17 \\
44.8 - 45.2 & 0.75 - 1.0 & 20.0 - 21.0 & -6.95 - -6.46 \\
44.8 - 45.2 & 0.75 - 1.0 & 21.0 - 22.0 & -7.15 - -6.55 \\
44.8 - 45.2 & 0.75 - 1.0 & 22.0 - 23.0 & -7.25 - -6.57 \\
44.8 - 45.2 & 0.75 - 1.0 & 23.0 - 23.5 & -7.23 - -6.40 \\
44.8 - 45.2 & 0.75 - 1.0 & 23.5 - 24.0 & -7.23 - -6.32 \\
44.8 - 45.2 & 0.75 - 1.0 & 24.0 - 26.0 & -7.19 - -6.16 \\
44.8 - 45.2 & 1.0 - 1.25 & 20.0 - 21.0 & -6.66 - -6.31 \\
44.8 - 45.2 & 1.0 - 1.25 & 21.0 - 22.0 & -6.95 - -6.50 \\
44.8 - 45.2 & 1.0 - 1.25 & 22.0 - 23.0 & -7.06 - -6.54 \\
44.8 - 45.2 & 1.0 - 1.25 & 23.0 - 23.5 & -7.01 - -6.37 \\
44.8 - 45.2 & 1.0 - 1.25 & 23.5 - 24.0 & -7.00 - -6.28 \\
44.8 - 45.2 & 1.0 - 1.25 & 24.0 - 26.0 & -6.99 - -6.13 \\
44.8 - 45.2 & 1.25 - 1.5 & 20.0 - 21.0 & -6.55 - -6.29 \\
44.8 - 45.2 & 1.25 - 1.5 & 21.0 - 22.0 & -6.75 - -6.43 \\
44.8 - 45.2 & 1.25 - 1.5 & 22.0 - 23.0 & -6.85 - -6.46 \\
44.8 - 45.2 & 1.25 - 1.5 & 23.0 - 23.5 & -6.81 - -6.29 \\
44.8 - 45.2 & 1.25 - 1.5 & 23.5 - 24.0 & -6.80 - -6.20 \\
44.8 - 45.2 & 1.25 - 1.5 & 24.0 - 26.0 & -6.77 - -6.06 \\
44.8 - 45.2 & 1.5 - 1.8 & 20.0 - 21.0 & -6.46 - -6.18 \\
44.8 - 45.2 & 1.5 - 1.8 & 21.0 - 22.0 & -6.60 - -6.30 \\
44.8 - 45.2 & 1.5 - 1.8 & 22.0 - 23.0 & -6.68 - -6.32 \\
44.8 - 45.2 & 1.5 - 1.8 & 23.0 - 23.5 & -6.64 - -6.17 \\
44.8 - 45.2 & 1.5 - 1.8 & 23.5 - 24.0 & -6.64 - -6.11 \\
44.8 - 45.2 & 1.5 - 1.8 & 24.0 - 26.0 & -6.62 - -5.97 \\
44.8 - 45.2 & 1.8 - 2.1 & 20.0 - 21.0 & -6.47 - -6.17 \\
44.8 - 45.2 & 1.8 - 2.1 & 21.0 - 22.0 & -6.54 - -6.26 \\
44.8 - 45.2 & 1.8 - 2.1 & 22.0 - 23.0 & -6.59 - -6.26 \\
44.8 - 45.2 & 1.8 - 2.1 & 23.0 - 23.5 & -6.52 - -6.13 \\
44.8 - 45.2 & 1.8 - 2.1 & 23.5 - 24.0 & -6.53 - -6.06 \\
44.8 - 45.2 & 1.8 - 2.1 & 24.0 - 26.0 & -6.50 - -5.93 \\
44.8 - 45.2 & 2.1 - 2.7 & 20.0 - 21.0 & -6.57 - -6.29 \\
44.8 - 45.2 & 2.1 - 2.7 & 21.0 - 22.0 & -6.60 - -6.30 \\
44.8 - 45.2 & 2.1 - 2.7 & 22.0 - 23.0 & -6.57 - -6.23 \\
44.8 - 45.2 & 2.1 - 2.7 & 23.0 - 23.5 & -6.52 - -6.11 \\
44.8 - 45.2 & 2.1 - 2.7 & 23.5 - 24.0 & -6.53 - -6.08 \\
44.8 - 45.2 & 2.1 - 2.7 & 24.0 - 26.0 & -6.51 - -5.96 \\
44.8 - 45.2 & 2.7 - 3.2 & 20.0 - 21.0 & -6.83 - -6.39 \\
44.8 - 45.2 & 2.7 - 3.2 & 21.0 - 22.0 & -6.77 - -6.35 \\
44.8 - 45.2 & 2.7 - 3.2 & 22.0 - 23.0 & -6.65 - -6.22 \\
44.8 - 45.2 & 2.7 - 3.2 & 23.0 - 23.5 & -6.60 - -6.12 \\
44.8 - 45.2 & 2.7 - 3.2 & 23.5 - 24.0 & -6.61 - -6.08 \\
44.8 - 45.2 & 2.7 - 3.2 & 24.0 - 26.0 & -6.59 - -5.96 \\
44.8 - 45.2 & 3.2 - 4.0 & 20.0 - 21.0 & -7.04 - -6.50 \\
44.8 - 45.2 & 3.2 - 4.0 & 21.0 - 22.0 & -6.96 - -6.44 \\
44.8 - 45.2 & 3.2 - 4.0 & 22.0 - 23.0 & -6.83 - -6.31 \\
44.8 - 45.2 & 3.2 - 4.0 & 23.0 - 23.5 & -6.77 - -6.19 \\
44.8 - 45.2 & 3.2 - 4.0 & 23.5 - 24.0 & -6.78 - -6.17 \\
44.8 - 45.2 & 3.2 - 4.0 & 24.0 - 26.0 & -6.78 - -6.08 \\
44.8 - 45.2 & 4.0 - 7.0 & 20.0 - 21.0 & -7.37 - -6.55 \\
44.8 - 45.2 & 4.0 - 7.0 & 21.0 - 22.0 & -7.30 - -6.52 \\
44.8 - 45.2 & 4.0 - 7.0 & 22.0 - 23.0 & -7.18 - -6.45 \\
44.8 - 45.2 & 4.0 - 7.0 & 23.0 - 23.5 & -7.14 - -6.30 \\
44.8 - 45.2 & 4.0 - 7.0 & 23.5 - 24.0 & -7.14 - -6.26 \\
44.8 - 45.2 & 4.0 - 7.0 & 24.0 - 26.0 & -7.13 - -6.19 \\
\end{tabular}\newpage
\begin{tabular}{l l l | l}
$\log L$ & $z$ & $\log N_H$ & $\log \phi$ \\
\hline
45.2 - 45.6 & 0.001 - 0.1 & 20.0 - 21.0 & -8.54 - -6.45 \\
45.2 - 45.6 & 0.001 - 0.1 & 21.0 - 22.0 & -8.54 - -6.43 \\
45.2 - 45.6 & 0.001 - 0.1 & 22.0 - 23.0 & -8.51 - -6.38 \\
45.2 - 45.6 & 0.001 - 0.1 & 23.0 - 23.5 & -8.52 - -6.34 \\
45.2 - 45.6 & 0.001 - 0.1 & 23.5 - 24.0 & -8.50 - -6.30 \\
45.2 - 45.6 & 0.001 - 0.1 & 24.0 - 26.0 & -8.52 - -6.22 \\
45.2 - 45.6 & 0.1 - 0.3 & 20.0 - 21.0 & -8.42 - -6.52 \\
45.2 - 45.6 & 0.1 - 0.3 & 21.0 - 22.0 & -8.41 - -6.51 \\
45.2 - 45.6 & 0.1 - 0.3 & 22.0 - 23.0 & -8.41 - -6.48 \\
45.2 - 45.6 & 0.1 - 0.3 & 23.0 - 23.5 & -8.42 - -6.41 \\
45.2 - 45.6 & 0.1 - 0.3 & 23.5 - 24.0 & -8.43 - -6.36 \\
45.2 - 45.6 & 0.1 - 0.3 & 24.0 - 26.0 & -8.43 - -6.32 \\
45.2 - 45.6 & 0.3 - 0.5 & 20.0 - 21.0 & -8.18 - -6.61 \\
45.2 - 45.6 & 0.3 - 0.5 & 21.0 - 22.0 & -8.23 - -6.62 \\
45.2 - 45.6 & 0.3 - 0.5 & 22.0 - 23.0 & -8.26 - -6.58 \\
45.2 - 45.6 & 0.3 - 0.5 & 23.0 - 23.5 & -8.27 - -6.48 \\
45.2 - 45.6 & 0.3 - 0.5 & 23.5 - 24.0 & -8.26 - -6.44 \\
45.2 - 45.6 & 0.3 - 0.5 & 24.0 - 26.0 & -8.25 - -6.40 \\
45.2 - 45.6 & 0.5 - 0.75 & 20.0 - 21.0 & -7.98 - -6.73 \\
45.2 - 45.6 & 0.5 - 0.75 & 21.0 - 22.0 & -8.04 - -6.74 \\
45.2 - 45.6 & 0.5 - 0.75 & 22.0 - 23.0 & -8.11 - -6.71 \\
45.2 - 45.6 & 0.5 - 0.75 & 23.0 - 23.5 & -8.11 - -6.59 \\
45.2 - 45.6 & 0.5 - 0.75 & 23.5 - 24.0 & -8.11 - -6.54 \\
45.2 - 45.6 & 0.5 - 0.75 & 24.0 - 26.0 & -8.09 - -6.46 \\
45.2 - 45.6 & 0.75 - 1.0 & 20.0 - 21.0 & -7.71 - -6.75 \\
45.2 - 45.6 & 0.75 - 1.0 & 21.0 - 22.0 & -7.84 - -6.81 \\
45.2 - 45.6 & 0.75 - 1.0 & 22.0 - 23.0 & -7.93 - -6.79 \\
45.2 - 45.6 & 0.75 - 1.0 & 23.0 - 23.5 & -7.94 - -6.62 \\
45.2 - 45.6 & 0.75 - 1.0 & 23.5 - 24.0 & -7.90 - -6.58 \\
45.2 - 45.6 & 0.75 - 1.0 & 24.0 - 26.0 & -7.91 - -6.47 \\
45.2 - 45.6 & 1.0 - 1.25 & 20.0 - 21.0 & -7.48 - -6.71 \\
45.2 - 45.6 & 1.0 - 1.25 & 21.0 - 22.0 & -7.67 - -6.83 \\
45.2 - 45.6 & 1.0 - 1.25 & 22.0 - 23.0 & -7.76 - -6.81 \\
45.2 - 45.6 & 1.0 - 1.25 & 23.0 - 23.5 & -7.75 - -6.66 \\
45.2 - 45.6 & 1.0 - 1.25 & 23.5 - 24.0 & -7.73 - -6.60 \\
45.2 - 45.6 & 1.0 - 1.25 & 24.0 - 26.0 & -7.72 - -6.45 \\
45.2 - 45.6 & 1.25 - 1.5 & 20.0 - 21.0 & -7.38 - -6.79 \\
45.2 - 45.6 & 1.25 - 1.5 & 21.0 - 22.0 & -7.52 - -6.83 \\
45.2 - 45.6 & 1.25 - 1.5 & 22.0 - 23.0 & -7.62 - -6.81 \\
45.2 - 45.6 & 1.25 - 1.5 & 23.0 - 23.5 & -7.62 - -6.65 \\
45.2 - 45.6 & 1.25 - 1.5 & 23.5 - 24.0 & -7.59 - -6.58 \\
45.2 - 45.6 & 1.25 - 1.5 & 24.0 - 26.0 & -7.56 - -6.42 \\
45.2 - 45.6 & 1.5 - 1.8 & 20.0 - 21.0 & -7.31 - -6.78 \\
45.2 - 45.6 & 1.5 - 1.8 & 21.0 - 22.0 & -7.42 - -6.80 \\
45.2 - 45.6 & 1.5 - 1.8 & 22.0 - 23.0 & -7.52 - -6.80 \\
45.2 - 45.6 & 1.5 - 1.8 & 23.0 - 23.5 & -7.49 - -6.61 \\
45.2 - 45.6 & 1.5 - 1.8 & 23.5 - 24.0 & -7.47 - -6.54 \\
45.2 - 45.6 & 1.5 - 1.8 & 24.0 - 26.0 & -7.43 - -6.37 \\
45.2 - 45.6 & 1.8 - 2.1 & 20.0 - 21.0 & -7.30 - -6.76 \\
45.2 - 45.6 & 1.8 - 2.1 & 21.0 - 22.0 & -7.37 - -6.77 \\
45.2 - 45.6 & 1.8 - 2.1 & 22.0 - 23.0 & -7.43 - -6.78 \\
45.2 - 45.6 & 1.8 - 2.1 & 23.0 - 23.5 & -7.40 - -6.58 \\
45.2 - 45.6 & 1.8 - 2.1 & 23.5 - 24.0 & -7.39 - -6.50 \\
45.2 - 45.6 & 1.8 - 2.1 & 24.0 - 26.0 & -7.36 - -6.36 \\
45.2 - 45.6 & 2.1 - 2.7 & 20.0 - 21.0 & -7.35 - -6.80 \\
45.2 - 45.6 & 2.1 - 2.7 & 21.0 - 22.0 & -7.39 - -6.80 \\
45.2 - 45.6 & 2.1 - 2.7 & 22.0 - 23.0 & -7.41 - -6.74 \\
45.2 - 45.6 & 2.1 - 2.7 & 23.0 - 23.5 & -7.38 - -6.55 \\
45.2 - 45.6 & 2.1 - 2.7 & 23.5 - 24.0 & -7.38 - -6.46 \\
45.2 - 45.6 & 2.1 - 2.7 & 24.0 - 26.0 & -7.34 - -6.37 \\
45.2 - 45.6 & 2.7 - 3.2 & 20.0 - 21.0 & -7.53 - -6.78 \\
45.2 - 45.6 & 2.7 - 3.2 & 21.0 - 22.0 & -7.52 - -6.74 \\
45.2 - 45.6 & 2.7 - 3.2 & 22.0 - 23.0 & -7.46 - -6.66 \\
45.2 - 45.6 & 2.7 - 3.2 & 23.0 - 23.5 & -7.43 - -6.51 \\
45.2 - 45.6 & 2.7 - 3.2 & 23.5 - 24.0 & -7.43 - -6.44 \\
45.2 - 45.6 & 2.7 - 3.2 & 24.0 - 26.0 & -7.41 - -6.35 \\
45.2 - 45.6 & 3.2 - 4.0 & 20.0 - 21.0 & -7.70 - -6.81 \\
45.2 - 45.6 & 3.2 - 4.0 & 21.0 - 22.0 & -7.66 - -6.76 \\
45.2 - 45.6 & 3.2 - 4.0 & 22.0 - 23.0 & -7.61 - -6.67 \\
45.2 - 45.6 & 3.2 - 4.0 & 23.0 - 23.5 & -7.56 - -6.54 \\
45.2 - 45.6 & 3.2 - 4.0 & 23.5 - 24.0 & -7.56 - -6.48 \\
45.2 - 45.6 & 3.2 - 4.0 & 24.0 - 26.0 & -7.54 - -6.42 \\
45.2 - 45.6 & 4.0 - 7.0 & 20.0 - 21.0 & -7.96 - -6.82 \\
45.2 - 45.6 & 4.0 - 7.0 & 21.0 - 22.0 & -7.93 - -6.79 \\
45.2 - 45.6 & 4.0 - 7.0 & 22.0 - 23.0 & -7.87 - -6.71 \\
45.2 - 45.6 & 4.0 - 7.0 & 23.0 - 23.5 & -7.84 - -6.56 \\
45.2 - 45.6 & 4.0 - 7.0 & 23.5 - 24.0 & -7.84 - -6.52 \\
45.2 - 45.6 & 4.0 - 7.0 & 24.0 - 26.0 & -7.81 - -6.50 \\
\end{tabular}\newpage
\begin{tabular}{l l l | l}
$\log L$ & $z$ & $\log N_H$ & $\log \phi$ \\
\hline
45.6 - 46.0 & 0.001 - 0.1 & 20.0 - 21.0 & -9.17 - -6.53 \\
45.6 - 46.0 & 0.001 - 0.1 & 21.0 - 22.0 & -9.16 - -6.51 \\
45.6 - 46.0 & 0.001 - 0.1 & 22.0 - 23.0 & -9.16 - -6.47 \\
45.6 - 46.0 & 0.001 - 0.1 & 23.0 - 23.5 & -9.15 - -6.41 \\
45.6 - 46.0 & 0.001 - 0.1 & 23.5 - 24.0 & -9.14 - -6.38 \\
45.6 - 46.0 & 0.001 - 0.1 & 24.0 - 26.0 & -9.15 - -6.33 \\
45.6 - 46.0 & 0.1 - 0.3 & 20.0 - 21.0 & -9.07 - -6.61 \\
45.6 - 46.0 & 0.1 - 0.3 & 21.0 - 22.0 & -9.06 - -6.58 \\
45.6 - 46.0 & 0.1 - 0.3 & 22.0 - 23.0 & -9.06 - -6.54 \\
45.6 - 46.0 & 0.1 - 0.3 & 23.0 - 23.5 & -9.07 - -6.49 \\
45.6 - 46.0 & 0.1 - 0.3 & 23.5 - 24.0 & -9.05 - -6.45 \\
45.6 - 46.0 & 0.1 - 0.3 & 24.0 - 26.0 & -9.07 - -6.42 \\
45.6 - 46.0 & 0.3 - 0.5 & 20.0 - 21.0 & -8.88 - -6.69 \\
45.6 - 46.0 & 0.3 - 0.5 & 21.0 - 22.0 & -8.89 - -6.69 \\
45.6 - 46.0 & 0.3 - 0.5 & 22.0 - 23.0 & -8.89 - -6.67 \\
45.6 - 46.0 & 0.3 - 0.5 & 23.0 - 23.5 & -8.90 - -6.57 \\
45.6 - 46.0 & 0.3 - 0.5 & 23.5 - 24.0 & -8.91 - -6.54 \\
45.6 - 46.0 & 0.3 - 0.5 & 24.0 - 26.0 & -8.92 - -6.53 \\
45.6 - 46.0 & 0.5 - 0.75 & 20.0 - 21.0 & -8.72 - -6.81 \\
45.6 - 46.0 & 0.5 - 0.75 & 21.0 - 22.0 & -8.74 - -6.82 \\
45.6 - 46.0 & 0.5 - 0.75 & 22.0 - 23.0 & -8.76 - -6.79 \\
45.6 - 46.0 & 0.5 - 0.75 & 23.0 - 23.5 & -8.78 - -6.66 \\
45.6 - 46.0 & 0.5 - 0.75 & 23.5 - 24.0 & -8.78 - -6.63 \\
45.6 - 46.0 & 0.5 - 0.75 & 24.0 - 26.0 & -8.77 - -6.63 \\
45.6 - 46.0 & 0.75 - 1.0 & 20.0 - 21.0 & -8.53 - -6.89 \\
45.6 - 46.0 & 0.75 - 1.0 & 21.0 - 22.0 & -8.57 - -6.89 \\
45.6 - 46.0 & 0.75 - 1.0 & 22.0 - 23.0 & -8.62 - -6.86 \\
45.6 - 46.0 & 0.75 - 1.0 & 23.0 - 23.5 & -8.64 - -6.74 \\
45.6 - 46.0 & 0.75 - 1.0 & 23.5 - 24.0 & -8.62 - -6.70 \\
45.6 - 46.0 & 0.75 - 1.0 & 24.0 - 26.0 & -8.61 - -6.68 \\
45.6 - 46.0 & 1.0 - 1.25 & 20.0 - 21.0 & -8.36 - -6.93 \\
45.6 - 46.0 & 1.0 - 1.25 & 21.0 - 22.0 & -8.43 - -6.95 \\
45.6 - 46.0 & 1.0 - 1.25 & 22.0 - 23.0 & -8.49 - -6.91 \\
45.6 - 46.0 & 1.0 - 1.25 & 23.0 - 23.5 & -8.50 - -6.80 \\
45.6 - 46.0 & 1.0 - 1.25 & 23.5 - 24.0 & -8.48 - -6.74 \\
45.6 - 46.0 & 1.0 - 1.25 & 24.0 - 26.0 & -8.47 - -6.68 \\
45.6 - 46.0 & 1.25 - 1.5 & 20.0 - 21.0 & -8.28 - -6.98 \\
45.6 - 46.0 & 1.25 - 1.5 & 21.0 - 22.0 & -8.34 - -6.98 \\
45.6 - 46.0 & 1.25 - 1.5 & 22.0 - 23.0 & -8.40 - -6.94 \\
45.6 - 46.0 & 1.25 - 1.5 & 23.0 - 23.5 & -8.40 - -6.82 \\
45.6 - 46.0 & 1.25 - 1.5 & 23.5 - 24.0 & -8.37 - -6.75 \\
45.6 - 46.0 & 1.25 - 1.5 & 24.0 - 26.0 & -8.35 - -6.67 \\
45.6 - 46.0 & 1.5 - 1.8 & 20.0 - 21.0 & -8.22 - -7.01 \\
45.6 - 46.0 & 1.5 - 1.8 & 21.0 - 22.0 & -8.29 - -7.00 \\
45.6 - 46.0 & 1.5 - 1.8 & 22.0 - 23.0 & -8.31 - -6.98 \\
45.6 - 46.0 & 1.5 - 1.8 & 23.0 - 23.5 & -8.33 - -6.81 \\
45.6 - 46.0 & 1.5 - 1.8 & 23.5 - 24.0 & -8.30 - -6.76 \\
45.6 - 46.0 & 1.5 - 1.8 & 24.0 - 26.0 & -8.27 - -6.65 \\
45.6 - 46.0 & 1.8 - 2.1 & 20.0 - 21.0 & -8.21 - -7.06 \\
45.6 - 46.0 & 1.8 - 2.1 & 21.0 - 22.0 & -8.24 - -7.04 \\
45.6 - 46.0 & 1.8 - 2.1 & 22.0 - 23.0 & -8.28 - -7.01 \\
45.6 - 46.0 & 1.8 - 2.1 & 23.0 - 23.5 & -8.27 - -6.82 \\
45.6 - 46.0 & 1.8 - 2.1 & 23.5 - 24.0 & -8.25 - -6.77 \\
45.6 - 46.0 & 1.8 - 2.1 & 24.0 - 26.0 & -8.22 - -6.65 \\
45.6 - 46.0 & 2.1 - 2.7 & 20.0 - 21.0 & -8.22 - -7.10 \\
45.6 - 46.0 & 2.1 - 2.7 & 21.0 - 22.0 & -8.24 - -7.09 \\
45.6 - 46.0 & 2.1 - 2.7 & 22.0 - 23.0 & -8.27 - -7.03 \\
45.6 - 46.0 & 2.1 - 2.7 & 23.0 - 23.5 & -8.25 - -6.84 \\
45.6 - 46.0 & 2.1 - 2.7 & 23.5 - 24.0 & -8.23 - -6.77 \\
45.6 - 46.0 & 2.1 - 2.7 & 24.0 - 26.0 & -8.23 - -6.64 \\
45.6 - 46.0 & 2.7 - 3.2 & 20.0 - 21.0 & -8.30 - -7.05 \\
45.6 - 46.0 & 2.7 - 3.2 & 21.0 - 22.0 & -8.30 - -7.03 \\
45.6 - 46.0 & 2.7 - 3.2 & 22.0 - 23.0 & -8.31 - -6.96 \\
45.6 - 46.0 & 2.7 - 3.2 & 23.0 - 23.5 & -8.30 - -6.79 \\
45.6 - 46.0 & 2.7 - 3.2 & 23.5 - 24.0 & -8.27 - -6.71 \\
45.6 - 46.0 & 2.7 - 3.2 & 24.0 - 26.0 & -8.27 - -6.58 \\
45.6 - 46.0 & 3.2 - 4.0 & 20.0 - 21.0 & -8.40 - -7.04 \\
45.6 - 46.0 & 3.2 - 4.0 & 21.0 - 22.0 & -8.39 - -7.01 \\
45.6 - 46.0 & 3.2 - 4.0 & 22.0 - 23.0 & -8.38 - -6.93 \\
45.6 - 46.0 & 3.2 - 4.0 & 23.0 - 23.5 & -8.39 - -6.77 \\
45.6 - 46.0 & 3.2 - 4.0 & 23.5 - 24.0 & -8.37 - -6.69 \\
45.6 - 46.0 & 3.2 - 4.0 & 24.0 - 26.0 & -8.33 - -6.61 \\
45.6 - 46.0 & 4.0 - 7.0 & 20.0 - 21.0 & -8.59 - -6.97 \\
45.6 - 46.0 & 4.0 - 7.0 & 21.0 - 22.0 & -8.59 - -6.95 \\
45.6 - 46.0 & 4.0 - 7.0 & 22.0 - 23.0 & -8.57 - -6.87 \\
45.6 - 46.0 & 4.0 - 7.0 & 23.0 - 23.5 & -8.56 - -6.72 \\
45.6 - 46.0 & 4.0 - 7.0 & 23.5 - 24.0 & -8.55 - -6.67 \\
45.6 - 46.0 & 4.0 - 7.0 & 24.0 - 26.0 & -8.55 - -6.65 \\
\end{tabular}\newpage

